Do Users Care about Ad's Performance Costs? Exploring the Effects of the Performance Costs of In-App Ads on User Experience

Context: In-app advertising is the primary source of revenue for many mobile apps. The cost of advertising (ad cost) is non-negligible for app developers to ensure a good user experience and continuous profits. Previous studies mainly focus on addressing the hidden performance costs generated by ads, including consumption of memory, CPU, data traffic, and battery. However, there is no research onanalyzing users' perceptions of ads' performance costs to our knowledge. Objective: To fill this gap and better understand the effects of performance costs of in-app ads on user experience, we conduct a study on analyzing user concerns about ads' performance costs. Method: First, we propose RankMiner, an approach to quantify user concerns about specific appissues, including performance costs. Then, based on the usage traces of 20 subject apps, we measure the performance costs of ads. Finally, we conduct correlation analysis on the performance costs and quantified user concerns to explore whether users complain more for higher performance costs. Results: Our findings include the following: (1) RankMiner can quantify users' concerns better than baselines by an improvement of 214% and 2.5% in terms of Pearson correlation coefficient (a metricfor computing correlations between two variables) and NDCG score (a metric for computing accuracyin prioritizing issues), respectively. (2) The performance costs of the with-ads versions are statistically significantly larger than those of no-ads versions with negligible effect size; (3) Users are moreconcerned about the battery costs of ads, and tend to be insensitive to ads' data traffic costs. Conclusion: Our study is complementary to previous work on in-app ads, and can encourage devel-opers to pay more attention to alleviating the most user-concerned performance costs, such as battery cost.

==> sections/analysis_review.tex <==
\subsection{Major Ad Issues Concerned by Users}
\noindent \textbf{Methodology:} We first retrieve \textbf{ad-related reviews} by extracting the reviews explicitly related to ads, \textit{i.e.}, reviews containing words such as ``ad'', ``ads'', or ``advert*'' (with regular expression), following the method by~\citet{gui2015truth}. We then use the third step in RankMiner to identify ad-related issues. Specifically, we retrieve top 50 (i.e., $k$=50) terms most similar to the words ``ad'' or ``ads''. The retrieved ad-related words are finally manually clustered.

To better illustrate the ad issues, we visualize them into a bubble graph. Each term corresponds to a bubble, and the distance between two bubble centers represent the cosine distance of their vector representations. We use bubble sizes to denote the quantified user concern regarding each term following the method in Section~\ref{issue_detection}, and implement the visualization based on gensim~\citep{rehurek_lrec} and Google Chart~\citep{googlecharts}.


\begin{figure}
	\centering
	\includegraphics[width=0.47 \textwidth]{figs//ad_visualize.PNG}
	\captionsetup{aboveskip=-0.2ex}
	\caption{Visualization of ad issues. Different colors indicate different types of ad issues.}
	\label{fig:adissue}
\end{figure}

\noindent \textbf{Result:} We extract 19,579 ad-related reviews from the 2,637,438 Google Play reviews used in CrossMiner~\citep{man2016experience}, and identify 22 ad-related terms which are manually clustered into five types of ad issues. The ad issue types include obstruction, ad size, ad timing, appearing style, and ad content. Figure~\ref{fig:adissue} shows the details of each ad issue type, and larger bubbles indicate that the corresponding issues are of more concern to users. In the following, we elaborate on the five types of ad issues using user reviews.

\textit{\textbf{Ad Content:}} Based on the review analysis, we discover that ad contents receive the highest concerns (64.0\%) from users, \textit{e.g.}, reviews with ``spam'' occupy 59.9\% of the ad review collection. This indicates that ads with junk or unwanted information are likely to receive unfavorable user feedback. For example, users complain about ``Annoying ad and notification spam.'' for the app \textit{com.myfitnesspal.android}, and ``Spam bogus ad is annoying.'' for the app \textit{com.droid27.transparentclockweather}. When users are frequently shown irrelevant ads, they tend to uninstall the apps. According to the study~\citep{DBLP:conf/mobisys/NathLRP13}, ad displaying without considering the content of the page or user preference is one key reason for reduced users' dwell time on ads, and declining developers' ad benefits. For example, displaying gambling ads in a bible app is not uncommon for users. Thus, developers should choose ad SDKs good at recommending relevant ads.

\textit{\textbf{Appearance style:}} The appearance styles of ads, such as popping up, significantly influence users' acceptance of ads. Annoyed users may post negative reviews with terms, such as ``ad pop up'', ``pop up ad'', and ``popups'', which account for 14.7\% of all ad issues. For example, one user complains that ``The same reviews repeat all the time, especially the pop-up ad is very annoying.'' (bbc.mobile.news.ww). Such ads can interfere with the user experience of the apps, since pop-up ads may interrupt users' interactions with apps and generate inadvertent clicks on the ads. This is reflected in that ``click bait'', whose main purpose is to attract users to click and visit particular web pages, is close to the issue of ``popups'' in Figure~\ref{fig:adissue}. Thus, developers should avoid embedding pop-up ads into apps.

\textit{\textbf{Ad Size:}} Generally, developers are required to define the ad display sizes, mainly including full-screen ads (\textit{i.e.}, interstitials) and banner ads (\textit{i.e.}, banners). As Figure~\ref{fig:adissue} depicts, the issues related to ad sizes, represented as red bubbles, occupy a certain proportion of all the ad-related issues (3.7\%). The negative reviews about ad sizes are usually described with terms like ``banner ad'' and ``full screen ad''. We also discover that the ``full screen ad'' is more concerned by users than ``banner ads'' (0.7\% more), which implies that full screen ads are more disruptive to users. Interstitials with unobservable closing buttons may provoke users to uninstall the apps. Hence, developers should choose ads with appropriate sizes and visible closing symbols.

\textit{\textbf{Ad timing:}} Ad timing refers to a particular ad display time that users cannot skip. This kind of ad issues mainly occurs with video ads and occupies 3.0\% of all ad issues. Users are compelled to view ads at the beginning or end of an activity without any skipping choices, which may cause discontents in users. Annoyed users may express this with ``unskippable'', ``30 second ads'', ``15 second ad'' and other terms with time settings in reviews. For example, one review mentions ``A 15 seconds ad play before any video content which is really annoying.'' (bbc.mobile.news.ww). Moreover, these ads are not skippable, reflected in the reviews like ``The ad is most annoying as they are repetitive and there is no way to skip them.'' (bbc.mobile.news.ww) and ``Shouldn't force to watch the same 30 seconds ad over and over without option to skip ads.'' (con.foxnews.android). Thus, developers should display short video ads in apps and provide users with skip permissions.

\textit{\textbf{Obstruction:}} Previous work~\citep{aduninstall} shows that almost 50\% of users uninstall apps just because of intrusive advertisement. In Figure~\ref{fig:adissue}, the characteristics of such obstruction are reflected in terms such as ``intrusive ad'', ``obtrusive'', and ``obnoxious ad''. This type of ad issues occupies a large proportion (14.7\%) of all the ad issues. As Figure~\ref{fig:adissue} shows, terms related to ``obstruction'' are close to those related to the appearance style of ads (``popups''), ad contents (``spam''), ad timing (``30 second ads''), and ad sizes (``full screen ad''). This indicates that all the ad issues above are correlated with the ``obstruction'' feature of ads. Developers should therefore pay much attention to ad design and provide user-friendly mobile advertisement that does not interfere with the user experience.

==> sections/case.tex <==
\section{Developer Survey}\label{sec:case}
To validate whether our insights are endorsed by developers, we conduct a survey of engineers from Microsoft. We collect 87 survey feedback in total. We focus on analyzing the answers of those participants who answered that they have app development experience (34/87). The participants include seven staff developers, 24 interns, and three researchers. 15 (44.1\%) of them have designed more than one app (for Android, iOS, or Windows Phone Systems) and 19 (55.9\%) of them have experience in designing one app. The user study is conducted through an online questionnaire, which consists of four questions: two questions on the participant's background, one question as a transitional inquiry and about in-app advertising, and one question (including five multiple-choice questions) for assessing of our advertising insights 2$\sim$6. Table~\ref{tab:survey} depicts the questions of the survey, as well as the aggregated data regarding the answers provided by the participants.


\begin{table}
	\center
	\caption{Survey data.}
	\label{tab:survey}
	\scalebox{0.64}{\begin{tabular}{|L{22em}|l|r|}
		%\rowcolor{gray!50}
		\hline
		Question & \multicolumn{2}{l|}{Answer} \\
		\hline
	    \multirow{5}{*}{\parbox{22em}{1. What is your role in  software development? }}
	     & Development engineer & 7 (20.6\%)\\
		 & Product manager & 0 (0\%)\\
		 & Maintenance engineer & 0 (0\%)\\
		 & Intern & 24 (70.6\%)\\
		 & Researcher & 3 (8.8\%) \\
		 \hline
		 \multirow{3}{*}{\parbox{22em}{2. How many mobile apps have you ever created for Android/iOS/Windows phone/etc. phones?}} 
		 & More than one & 15 (44.1\%)\\
		 & Only One & 19 (55.9\%) \\
		 & Zero & 0 (0\%) \\
		 \hline
		 \multirow{3}{*}{\parbox{22em}{3. How do you think about in-app ads can bring benefits to developers?}} & Definitely can & 9 (26.5\%)\\
		 & Possibly, but with cost & 24 (70.6\%)\\
		 & Impossibly & 1 (2.9\%)\\
		 \hline
		 \multirow{3}{*}{\parbox{22em}{4. What do you think about the suggestion of recommending relevant ads for app development?}} & Reasonable & 25 (73.5\%)\\
		 & Practical & 9 (26.5\%)\\
		 & Novel & 3 (8.8\%)\\
		 \hline
		 \multirow{3}{*}{\parbox{22em}{5. What do you think about the suggestion of avoiding pop-up ads for app development?}} & Reasonable & 29 (85.3\%)\\
		 & Practical & 8 (23.5\%)\\
		 & Novel & 0 (0\%)\\
         \hline
         \multirow{3}{*}{\parbox{22em}{6. What do you think about the suggestion of avoiding full-screen ads and choosing appropriate ad sizes?}} & Reasonable & 26 (76.5\%)\\
		 & Practical & 11 (32.4\%)\\
		 & Novel & 0 (0\%)\\
		 \hline
		 \multirow{3}{*}{\parbox{22em}{7. What do you think about the suggestion of shortening ad displaying time for app development?}} & Reasonable & 25 (73.5\%)\\
		 & Practical & 13 (38.2\%)\\
		 & Novel & 5 (5.9\%)\\
        \hline
        \multirow{3}{*}{\parbox{22em}{8. What do you think about the finding that users pay little attention to memory/CPU/network cost of ads, but more care about the battery cost?}} & Reasonable & 21 (61.8\%)\\
		 & Practical & 11 (32.4\%)\\
		 & Novel & 7 (20.6\%)\\
		\hline
	\end{tabular}
}
\end{table}

The insights are assessed via three metrics: rationality, usefulness, and novelty, where novelty indicates whether the suggestions are instructive and rarely noticed before. Insights 1$\sim$5 correspond to the five small questions (Q4$\sim$Q8 in Table~\ref{tab:survey}), with results shown in Figure~\ref{fig:userstudy}. As the results indicate, more than half respondents agree with the rationality of the insights, with Insight 3 (\textit{i.e.}, avoiding pop-up ads) having the highest endorsement (85.3\%). Also, these insights are deemed useful by 26.5\%, 23.5\%, 32.4\%, 38.2\%, and 32.4\% of them, respectively. Interestingly, the novelty of Insight 6 (\textit{i.e.}, users tend to pay little attention to the memory/CPU/network cost of ads) is recognized by 20.6\% of participants. In addition, 91.2\% (31/34) of participants give positive feedback and consider these insights to be either rational, useful, or novel. Overall, our insights can not only inspire developers, but also provide guidance on in-app advertising. These results strengthen the validation of our suggestions.


%, while the insights 3-4 are not considered to be innovative (0\%) for them

\begin{figure}
	\centering
	\includegraphics[width=0.35 \textwidth]{figs//insight.pdf}
	\caption{Insight validation. Insight 1 suggests that developers should choose ad SDKs with good performance in recommending relevant ads to users. Insight 2 is about avoiding pop-up ads. Insight 3 is related to avoiding full-screen ads and providing obvious closing symbols in ads. Insight 4 suggests to shorten the compulsory video ads. Insight 5 summarizes that users are most concerned about the battery cost of ads, and tend to pay little attention to ads' memory, CPU, and network cost.}
	\label{fig:userstudy}
\end{figure}
